Video-kMaX: A Simple Unified Approach for Online and Near-Online Video Panoptic Segmentation

Video Panoptic Segmentation (VPS) aims to achieve comprehensive pixel-level scene understanding by segmenting all pixels and associating objects in a video. Current solutions can be categorized into online and near-online approaches. Evolving over the time, each category has its own specialized designs, making it nontrivial to adapt models between different categories. To alleviate the discrepancy, in this work, we propose a unified approach for online and near-online VPS. The meta architecture of the proposed Video-kMaX consists of two components: within clip segmenter (for clip-level segmentation) and cross-clip associater (for association beyond clips). We propose clip-kMaX (clip k-means mask transformer) and HiLA-MB (Hierarchical Location-Aware Memory Buffer) to instantiate the segmenter and associater, respectively. Our general formulation includes the online scenario as a special case by adopting clip length of one. Without bells and whistles, Video-kMaX sets a new state-of-the-art on KITTI-STEP and VIPSeg for video panoptic segmentation, and VSPW for video semantic segmentation. Code will be made publicly available.

==> sections/6.supple.tex <==
% \section{Additional analysis on $\lambda$}
% We provide an additional analysis on the hyper-parameter related to the appearance feature: $\lambda$, which balances the weight between the stored appearance feature in memory and the current one (see Eq.~(3) in the main paper). 
% The higher value of $\lambda$, the more weight will be given to the current appearance feature.
% In the extreme cases, $\lambda = 1$ means we will simply store the current appearance feature to the memory (\ie, not weighted average with the stored appearance feature), while $\lambda = 0$ means we will always use the appearance feature stored in the memory.
% We ablate it in a wide range from 0.0 up to 1.0 as shown in~\tabref{tab:ablation_lambda}.
% When it is set to 0.0, since we are not exploiting the current appearance feature, the association performance is downgraded.
% In a certain range of $\lambda$ (\eg, $0.7 - 0.9$), our \methodname robustly achieves the same result (74.22\% AQ). We choose 0.8 as a default value for our experiments.
% However, our \methodname robustly achieves same results in certain range from 0.7 to 0.9 of $\lambda$.
% As shown in~\tabref{tab:ablation_lambda}, our \methodname is robust to the different values of $\lambda$.
%% appearance lambda
% \input{tables/ablation_for_lambda}
%% algorithm

\section{Comparison with Normal Cross-Attention}
\label{sec:normal_cross_att}
As discussed in the Sec.~3.1 of main paper, we deliberately design our clip-$k$MaX with the $k$-means cross-attention~\cite{yu2022k}, which we empirically found to be very effective for handling the extremely large sequence of spatially and temporally flattened clip features.
We now elaborate on the experiments and particularly compare with the normal (\ie, original) cross-attention~\cite{vaswani2017attention} as well as the advanced latent memory cross-attention~\cite{kim2022tubeformer} (\ie, the cross-attention mechanism used in TubeFormer~\cite{kim2022tubeformer}, which adopts latent memory to facilitate attention learning between video frames).
% we intuitively claim that $k$-means cross attention better handles with the extremely large flattened clip features than normal cross attention due to the cluster-wise attention mechanism.

\tabref{tab:compare_cross} summarizes our findings.
To ensure the fairness, we employ the same backbone Axial-ResNet50-B1~\cite{wang2020axial} that has been pretrained on ImageNet-1K and Cityscapes.
The baseline, employing the normal cross-attention module, yields the performance of 68.4\% STQ.
The performance can be further improved by 1.6\% STQ, if we adopt the latent memory~\cite{kim2022tubeformer} in the cross-attention module.
By contrast, our clip-$k$MaX, adopting the $k$-means cross-attention mechanism, attains 73.9\% STQ, significantly outperforming the conventional cross-attention and latent memory cross-attention by {\bf +5.5\%} and {\bf +3.9\%} STQ, respectively.
The improvement is attributed to the effectiveness of $k$-means cross-attention that performs the cluster-wise argmax on cluster centers.
% In~\tabref{tab:compare_cross}, we empirically prove that $k$-means cross attention (clip-$k$MaX) outperforms normal cross attention by +10.1 AQ and 5.5 STQ, when both are utilized on the same Axial-ResNet50-B1 backbone that has been pretrained from ImageNet-1k and Cityscape. Additional methods for normal cross attention, for example, latent memory module and temporal-consistency, are also not able to improve the performance even close up to our clip-$k$MaX.
Additionally, we show that our proposed \methodname is complementary to clip-$k$MaX, which sets the best STQ performance (74.7 STQ). Our results suggest that using $k$-means cross-attention can reduce the ambiguity in cross-attention between queries and large flattened clip features, resulting in a higher quality of video panoptic segmentation results. 


\input{tables/compare_w_cross}

\input{tables/space_reduction}


\input{tables/flops_and_fps}


%% temperature
\input{tables/ablation_for_temperature}

%% appearance lambda
\input{tables/ablation_for_lambda}

\input{tables/algorithm}




\section{Analysis on Memory Matching Space}
\label{sec:analysis_memory_matching}
In the Sec.~3.2 of main paper, we address the limitations of the previous memory buffer approach~\cite{wu2022defense}, referred as na\"ive-MB.
One of the limitations of na\"ive-MB is the huge matching space in memory decoding, which increases the difficulty of matching and thus results in low association quality.
From that perspective, we empirically prove that our hierarchical matching scheme, \methodname, can effectively reduce the matching space size as shown in~\tabref{tab:space_reduction}.
To do so, we calculate the size of the similarity matrix $\mathbf{S}$ (\ie, $M\times N$, where there are $M$ objects in the memory and $N$ detected objects in the current frame) to quantitatively measure the matching space size.
We note that modern approaches~\cite{wu2022defense} adopt a memory refreshing strategy, where the old objects stored in the memory will be removed if they are $\tau$-frame older than the current frame, which, to some degree, alleviates the issue of large matching space.
However, we will show that using the memory refreshing strategy alone is not sufficient to reduce the matching space size.
We compare the matching space between na\"ive-MB and our \methodname under two cases of $\tau$, which is the hyper-parameter to refresh out the old objects in the memory, affecting the matching space size.
In the first case, we set $\tau$ to 1000, which mimics the ideal scenario where we have a very large memory and the old objects are barely removed, aiming to exclude the effect of refreshing strategy and focus on the memory buffer approach itself.
As shown in the table, we can observe that \methodname can greatly improve the matching space efficiency by a healthy margin (\ie, 3.4$\times$ smaller and 3.6$\times$ smaller in average and max values, respectively).
In the second case, $\tau$ is set to be the optimal value for each memory buffer approach (\ie, 1 for na\"ive-MB and 10 for \methodname).
As shown in the table, the memory refreshing strategy effectively reduces the matching space size for na\"ive-MB.
However, our \methodname still outperforms na\"ive-MB by achieving 9.1$\times$ and 8.2$\times$ more efficient matching space in average and max value, respectively.


\section{Analysis on Model Complexity}
\label{sec:analysis_model_complexity}
In~\tabref{tab:specs}, we measure params, FLOPs, and FPS for our method, using a Tesla V100 GPU with CUDA 11.0 and batch size $1$.
%We furnish a detailed account of the number of parameters, FLOPs (floating point operations), and FPS (frames per second) for different backbones and settings of our \modelname as shown in~\tabref{tab:specs}.
We run the inference 3 times to obtain the average and worst FPS.
%The statistics are measured on a Tesla V100 GPU with CUDA 11.0 and batch size $1$.
% We note that all the other existing methods do not report such statistics.
%Our backbones are Axial-ResNet50 and ConvNeXt-L.
% \vspace{-2.5mm}


\section{Algorithm for our \methodname}
\label{sec:algorithm_lamb}
In~\Aref{alg:pseudo}, we provide the algorithm for our \methodnamefull (\methodname), which consists of two phases: Encoding phase to store the previous object features, and Decoding phase to associate current objects with the objects stored in the
memory buffer. For better understanding, we also attach our code snippet in the supplementary materials.





\section{Feature-related Hyper-parameter}
\label{sec:feature_hyper}
% {\bf Feature-related hyper-parameter}~\quad
% In \equref{eqn:sim}, 
We adopt a temperature $T$ to scale the values between the location and appearance features (see Equ.~(5) of main paper).
As shown in~\tabref{tab:ablation_temperature}, our model is robust to the different values of $T$.
We thus default its value to 1 for simplicity.
Additionally, as shown in~\tabref{tab:ablation_lambda}, our model is also robust to the different values of $\lambda$, which balances the weight between the stored appearance feature in memory and the current one (see Equ.~(3) of main paper).

% (\equref{eq:mb_appearance_feature})

% In~\equref{eqn:sim}, we adopt a temperature $T$ to scale the values between the location and appearance features.
% As shown in~\tabref{tab:ablation_temperature}, our model is robust to the different values of $T$.
% We thus default its value to 1 for simplicity.
% Additionally, as shown in~\tabref{tab:ablation_lambda}, our model is also robust to the different values of $\lambda$ (\equref{eq:mb_appearance_feature}), which balances the weight between the stored appearance feature in memory and current one.


%%%%%%%%%%%%%%%%%%%%%%%%%% visulization  %%%%%%%%%%%%%%%%%%%%5
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\linewidth]{figs/pdf_folder/query_space.pdf}
% \includegraphics[bb=10 10 10 10]{figure/fig_arch/Teaser_v14.pdf}
% \vspace{1.0mm}
\caption{
{\bf Query Visualization} on KITTI-STEP \textit{val} set. We use \modelname with Axial-ResNet50-B1 backbone that is trained on KITTI-STEP and then plot the location of averaged mask center (including all stuff and things) predicted by each query.  
}
\label{fig:query_space}
\end{center}
\vspace{-0mm}
\end{figure}


\section{Visualization Anaylsis}
\label{sec:vis_analysis}

\paragraph{More qualitative results}
We show some visualization results in~\figref{fig:vip_seg_vis} for VIPSeg, where the baseline na\"ive-MB fails to associate persons in a crowd, since they have similar appearance features.
On the other hand, our \methodname correctly associates the same person by effectively exploiting both the appearance and location features.
In our supplementary submission, we also include video panoptic segmentation results on the validation sets of KITTI-STEP~\cite{weber2021step} and VIPSeg~\cite{miao2022large}.
Our \modelname (consisting of clip-$k$MaX and \methodname) demonstrates more clear and consistent video results than the baselines.

% %%%%%%%%%%%%%%%%%%%%%%%%%% visulization  %%%%%%%%%%%%%%%%%%%%5
\begin{figure*}[!th]
\begin{center}
\includegraphics[width=0.9\linewidth]{figs/pdf_folder/vip_seg_visual_v3.pdf}
% \includegraphics[bb=10 10 10 10]{figure/fig_arch/Teaser_v14.pdf}
% \vspace{1.0mm}
\caption{
{\bf Visualization results} on VIPSeg \textit{val} set.
The baseline na\"ive-MB, only exploiting the appearance feature, fails to associate the same person, as neighboring people have similar appearance features.
On the other hand, our \methodname, exploiting both appearance and location features, successfully associates the same person.
}
\label{fig:vip_seg_vis}
\end{center}
\vspace{-1mm}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%% visualization  %%%%%%%%%%%%%%%%%%%%5
\begin{figure*}[!th]
\begin{center}
\includegraphics[width=0.85\linewidth]{figs/pdf_folder/vip_seg_failure_v2.pdf}
% \includegraphics[bb=10 10 10 10]{figure/fig_arch/Teaser_v14.pdf}
% \vspace{1.0mm}
\caption{
{\bf Failure case} on VIPSeg \textit{val} set.
The target object is initially assigned with ID 99.
Its ID switches to 107 and 108 in frame 3 and frame 4, respectively.
Our method fails to track the target object, because it is heavily occluded and moves at a large random pace, making both appearance and location features unreliable.
}
\label{fig:vip_seg_fail}
\end{center}
\vspace{-0mm}
\end{figure*}

\paragraph{Structural prior learned by queries}
We observe that the object queries learned by our \modelname demonstrate a structural prior that a particular query will respond to objects around a specific location on the image plane.
To visualize the structural prior, for each query, we compute the mean location center of all its segmented objects in the whole KITTI-STEP validation set, and show the scatter plot in~\figref{fig:query_space}.
As shown in the figure, each object query is responsible to segment objects around a specific location on the image plane.
Interestingly, the object queries are scattered mostly along a vertical and a horizontal line, showing the property of ego-centric car in KITTI-STEP, where the street-view images are collected by a driving car.






% In \cref{fig:query_space}, we show the scatter plot of the learned queries based on the locations of their corresponding objects in the whole KITTI-STEP video sequence. We can find out that each query is predicted at different location. Due to its spatial specialization, we can say that learned query itself has a structural prior. 

\paragraph{Failure case and Limitation}
We analyze the failure mode of our \modelname in~\figref{fig:vip_seg_fail}.
The first row and second row are video frames and corresponding video panoptic results with our \modelname, respectively. We  observe that a person initially assigned with ID number 99 until frame 2 is re-assigned with different ID numbers, \ie, 107 (in frame 3) and 108 (in frame 4).
The ID switch could be attributed to two reasons.
First, the appearance feature of the occluded person (\ie, person ID 107 in frame 3) is not reliable, as most of its discriminative appearance regions are occluded.
Second, the target object demonstrates a large random movement, violating our slow linear motion assumption encoded by the location feature.
% since location feature of \methodname predicts the bounding box in a linear fashion, the predicted bounding box of ID 99 can not properly capture the location of dynamic moving object as drawn in frame 3 and 4.
This failure case presents a challenging but interesting research direction to further improve our model by strengthening both appearance and location features.
% We consider them as limitations and set future research direction to strengthen both appearance and location features further.

% \section{Limitations}


==> tables/ablation_for_near_lamb_on_kitti_supple.tex <==

% \begin{table}[t]
% \centering
% \small
% \tablestyle{3pt}{1.1}
\resizebox{0.92\linewidth}{!}{
\begin{tabular}{l|ccc|cc|c}
               & \multicolumn{3}{c|}{association features}  &  &  & \\
method         & video-stitching    & appearance      & location        & SQ      & AQ      & STQ       \\
\hline

        & \checkmark    &    &             & 74.2  &  72.3 &  73.3        \\
        &     & \checkmark  &                & 74.2    &   71.4   &     72.8 \\
        &     &      & \checkmark      &    74.2  &  72.3    & 73.2      \\
\modelname        &     & \checkmark & \checkmark      &  74.2     &  73.8    & 74.0      \\
(near-online)        & \checkmark    & \checkmark &      &    74.2  &    72.1  &   73.2  \\
        &  \checkmark   &  & \checkmark  & 74.2     &   73.6   & 73.9     \\
        &  \baseline{\checkmark}    &  \baseline{\checkmark} & \baseline{\checkmark}      & \baseline{74.2}     &  \baseline{74.2}    & \baseline{74.2}      \\
\end{tabular}}
% \vspace{-.8em}
% \caption{..}
% \label{tab:abla_near_lamb_kitti}
% \vspace{-2mm}
% \end{table}


==> tables/ablation_for_online_lamb_on_kitti_supple.tex <==

% \begin{table}[t]
% \centering
% \small
% \tablestyle{3pt}{1.1}
\resizebox{0.92\linewidth}{!}{
\begin{tabular}{l|c|cc|cc|c}
                &   & \multicolumn{2}{c|}{association features} & & & \\
method & backbone  & appearance      & location        & SQ      & AQ      & STQ       \\
\hline
\multirow{8}{*}{$k$Max-DeepLab}
    & \multirow{4}{*}{ResNet50}   &     &                 &  75.0    & 10.0      & 27.3       \\
    &    & \checkmark    &                 &  75.0    & 33.8      &   50.4    \\
    &    &               & \checkmark       &   75.0   &   \textbf{72.0}   &   \textbf{73.5}   \\
\modelname    &    & \checkmark    & \checkmark       &   75.0   &   66.4   &   70.6   \\
    \cline{2-7}\cline{2-7}
(online)    &  \multirow{4}{*}{ConvNeXt-L}    &     &                 &  77.2  & 10.4      & 28.3      \\
    &    & \checkmark    &                 &  77.2    & 61.6      &   69.0    \\
    &    &               & \checkmark       &   77.2   &   74.0   &   75.6   \\
    &    & \baseline{\checkmark}    & \baseline{\checkmark}       &   \baseline{77.2}   &   \baseline{\textbf{75.7}}   &   \baseline{\textbf{76.5}}   \\
\end{tabular}}
% \vspace{-.8em}
% \caption{..}
% \label{tab:abla_online_lamb_kitti}
% \vspace{-2mm}
% \end{table}

==> tables/algorithm.tex <==
\begin{algorithm}[hbt!]
% \ce
\DontPrintSemicolon
\vspace{-0.5mm}
\caption{Algorithm for \methodname}
\label{alg:pseudo}
\KwIn{\\
1. \textbf{\methodname} = $\{(\hat{q}^{t-1}_{j}, \hat{b}^{t-1}_{j})\}_{j=1}^M$ with $M$ encoded objects until frame $t-1$.\\
2. Feature set ($q_{i}$, $b_{i}$) of \textbf{object $i$} in current frame $t$.\\
3. Panoptic map $P\in\Re^{H\times W}$ of previous frame $t-1$
}
% \textbf{Input}: Target data $x_{t}$ = ($x^{2D}_{t}$, $x^{3D}_{t}$), Source pre-trained model $F$=($F^{2D}$, $F^{3D}$) \\
% \Parameter{Momentum factor $\lambda$, pseudo label threshold $\theta^{(k)}$}
\KwOut{(updated ID of \textbf{object $i$}, updated \textbf{\methodname})}
% \textbf{Output}:  The model with adapted weights on target dataset $F$=($F^{2D}$, $F^
% {3D}$)\\
\Begin
{
    \textcolor{teal}{\# Decoding phase.} \\
    \If{Video-Stitch(object $i$ and $P$) $\le M$}
    {
        \textcolor{teal}{\# $k$ is the updated ID of object $i$.} \\
        $k$ $\leftarrow$ Video-Stitch(object $i$ and $P$) \\
        % $i$ $\leftarrow$ $k$ \\
    }
    \Else{
        
        $f(i,j) = e^{-\|b_{i} - \hat{b}_{j}\|^2/T} \cdot cos(q_{i}, 
        \hat{q}_{j})$ \\
        % $sim$ = $\{e^{-\|b_{i} - \hat{b}_{j}\|^2/T} \cdot cos(q_{i}, 
        % \hat{q}_{j})\}_{j=1}^M$ \\
        $r$ = $\argmax_M(f(i,j)_{j=1}^M)$ \\
        \If{$f(i,r)$ $\ge \alpha$}
        {
            $k$ $\leftarrow$ $r$
        }
        \Else{
            $k$ $\leftarrow$ $M+1$
        }
    }
    \textcolor{teal}{\# Encoding phase.} \\
    \If{$k$ $\le M$}
    {
        \textcolor{teal}{\# The object is tracked in the memory.} \\
        $\hat{q}^t_{k} =  (1-\lambda)\hat{q}^{t-1}_{k} + \lambda q_{i}$ \\
        $\hat{b}^{t}_{k} = b_{i}$ \\
        \For{$j\in \{1,...,k-1,k+1,...M\}$}
        {
            $\hat{q}^t_{j} = \hat{q}^{t-1}_{j}$ \\ 
            $\hat{b}^{t}_{j}  = \hat{b}^{t-1}_{j} + (\hat{b}^{t-1}_{j}-\hat{b}^{t-2}_{j})$ 
        }
    }
    \Else{
        \textcolor{teal}{\# The object is new.} \\
        $\hat{q}^t_{k} = q_{i}$ \\
        $\hat{b}^{t}_{k} = b_{i}$ \\ 
        \For{$j\in \{1,...,M\}$}
        {
            $\hat{q}^t_{j} = \hat{q}^{t-1}_{j}$ \\
            $\hat{b}^{t}_{j}  = \hat{b}^{t-1}_{j} + (\hat{b}^{t-1}_{j}-\hat{b}^{t-2}_{j})$ 
        }
    }
    return ($k$, updated \textbf{\methodname})
}
% \vspace{-1mm}
\end{algorithm}

==> tables/flops_and_fps.tex <==
\begin{table*}[t!]
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|c|c|c|r|c|c|c}
%task      & method          & frame resolution   & T        & params (M)  & FLOPs (B)    & runtime (FPS)   & training memory (G)   \\
 \multirow{2}{*}{method} & \multirow{2}{*}{backbone}         & \multirow{2}{*}{frame size}  & \multirow{2}{*}{scenario}        & \multirow{2}{*}{params}  & \multirow{2}{*}{FLOPs}    & \multicolumn{2}{c}{FPS}   \\
 \cline{7-8}
 & & & & & & average & worst \\
\shline
        \multirow{4}{*}{\modelname} & \multirow{4}{*}{ResNet50}    & \multirow{2}{*}{375$\times$1242 (KITTI-STEP)}     & Online (T=1)        &   56.4M     &  83G      & 41.2       & 40.8     \\
        &    &  & Near-online (T=2)               &  56.4M      &    167G       &  23.4 & 23.3 \\
        \cline{3-8}
        &     & \multirow{2}{*}{720p (VIPSeg)}     & Online  (T=1)      &  56.4M       & 162G         &  24.4   & 24.0        \\
        &     &  & Near-online  (T=2)      & 56.4M     &  324G       &   13.6   & 13.5       \\
        \hline
        
        \multirow{4}{*}{\modelname} & \multirow{4}{*}{Axial-ResNet50-B1}    & \multirow{2}{*}{375$\times$1242 (KITTI-STEP)}     & Online (T=1) &  74.2M & 118G & 31.0 & 30.8  \\
        &    &  & Near-online  (T=2)      &   74.2M     &   236G      &   17.2  & 17.0       \\
        \cline{3-8}
        &     & \multirow{2}{*}{720p (VIPSeg)}     & Online  (T=1)      &  74.2M        &    231G     & 18.2     & 18.2         \\
        &     &  & Near-online  (T=2)      & 74.2M         &     461G    & 9.9     & 9.8      \\
        \hline

        \multirow{4}{*}{\modelname} & \multirow{4}{*}{ConvNeXt-L}     & \multirow{2}{*}{375$\times$1242 (KITTI-STEP)}     & Online (T=1)       &   231.6M      & 370G        &    12.9 & 12.8        \\
        &     &  & Near-online  (T=2)      &     231.6M    & 740G       &     6.9  & 6.8      \\
        \cline{3-8}
        &     & \multirow{2}{*}{720p (VIPSeg)}     & Online  (T=1)      &    231.6M      & 715G & 7.0      & 6.9        \\
        &     &  & Near-online (T=2)       & 231.6M         &    1431G     &  3.7    & 3.7       \\
\end{tabular}}
% \vspace{-1.1em}
\caption{{
\textbf{Model complexity}.
We report the inference complexity of our \modelname in terms of params, FLOPs, and FPS (frames per second) on a V100 GPU, under both the online and near-online scenarios.
We report three backbones, including ResNet50, Axial-ResNet50-B1, and ConvNeXt-L, on both the KITTI-STEP and VIPSeg datasets.
% \scriptsize{375$\times$1242 and 720p correspond to the frame size of KITTI-STEP and VIPSeg-VPS respectively.}
}}
\label{tab:specs}
\end{table*}
% \vspace{-1.3em}

==> tables/ytvis_19_val.tex <==
\begin{table}[!t]
\centering
\small
\tablestyle{4.0pt}{1.1}
\begin{tabular}{l|c|ccc|cc}
        method         & T  & AP        & AP\textsubscript{50} & AP\textsubscript{75} & AR\textsubscript{1}  & AR\textsubscript{10}     \\
\shline
% \multirow{6}{*}{\parbox{1.2cm}{proposal\\based}}
        MaskTrack~\cite{Yang19ICCV}    & 2  & 31.8      & 53.0      & 33.6      & 33.2      & 37.6       \\
        SipMask~\cite{cao2020sipmask}  & 2  & 33.7      & 54.1      & 35.8      & 35.4      & 40.1       \\
        %&CompFeat~\cite{fu2020compfeat} & x  & 35.3      & 56.0      & 38.6      & 33.1      & 40.3       \\
        STEm-Seg~\cite{athar2020stem}  & 8  & 34.6      & 55.8      & 37.9      & 34.4      & 41.6        \\
        CrossVIS~\cite{yang2021crossover} 
                                        & 2  & 36.6      & 57.3      & 39.7      & 36.0      & 42.0       \\
        MaskProp~\cite{bertasius2020classifying}  
                                        & 13  & 46.6      & -         & 51.2      & 44.0         & 52.6 \\
        %                                & 13  & 42.5      & -         & 45.6      & -         & -          \\
        Seq Mask R-CNN~\cite{lin2021video}  
                                        & 36  & {\bf 47.6}      & {\bf 71.6}    & 51.8      & 46.3         & 56.0 \\
        
        VisTR~\cite{wang2021end}       & 36 & 40.1      & 64.0      & 45.0      & 38.3      & 44.9       \\
        IFC~\cite{hwang2021video}      & 36 & 44.6      & 69.2      & 49.5      & 44.0      & 52.1       \\

\hline
        TF-DL-B4                       & 5  & {47.5}  & 68.7      & \textbf{52.1}   & \textbf{50.2} & \textbf{59.0}  \\

\hline
\hline
        \modelname + LA-MB  & 5 & & & & &

        \\
\end{tabular}
\vspace{-.8em}
\caption{\textbf{[VIS]} YouTube-VIS-2019 {\it val} set results. \shin{show the backbone as well}
}
\label{tab:yt_vis_19}
\vspace{-1mm}
\end{table}
